Stationary Velocity Fields on Matrix Groups for Deformable Image Registration

The stationary velocity field (SVF) approach allows to build parametrizations of invertible deformation fields, which is often a desirable property in image registration. Its expressiveness is particularly attractive when used as a block following a machine learning-inspired network. However, it can struggle with large deformations. We extend the SVF approach to matrix groups, in particular $\SE(3)$. This moves Euclidean transformations into the low-frequency part, towards which network architectures are often naturally biased, so that larger motions can be recovered more easily. This requires an extension of the flow equation, for which we provide sufficient conditions for existence. We further prove a decomposition condition that allows us to apply a scaling-and-squaring approach for efficient numerical integration of the flow equation. We numerically validate the approach on inter-patient registration of 3D MRI images of the human brain.

==> plots/TikzPictures/bigpicture.tex <==
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{fadings}
\usetikzlibrary{fit}
\definecolor{fc}{HTML}{1E90FF}
\definecolor{h}{HTML}{228B22}
\definecolor{bias}{HTML}{87CEFA}
\definecolor{noise}{HTML}{8B008B}
\definecolor{conv}{HTML}{b6e1fc}
\definecolor{cyan}{HTML}{87CEFA}
\definecolor{pool}{HTML}{098bdc}
\definecolor{up}{HTML}{B22222}
\definecolor{view}{HTML}{FFFFFF}
\definecolor{bn}{HTML}{FFD700}
\tikzset{fc/.style={black,draw=black,fill=fc,rectangle,minimum height=1cm}}
\tikzset{h/.style={black,draw=black,fill=h,rectangle,minimum height=1cm}}
\tikzset{bias/.style={black,draw=black,fill=bias,rectangle,minimum height=1cm}}
\tikzset{noise/.style={black,draw=black,fill=noise,rectangle,minimum height=1cm}}
\tikzset{conv/.style={black,draw=black,fill=conv,rectangle,minimum height=1cm}}
\tikzset{block/.style={black,draw=black,fill=conv,fill opacity=0.95,rectangle,minimum height=1cm}}
\tikzset{pool/.style={black,draw=black,fill=pool,rectangle,minimum height=1cm}}
\tikzset{up/.style={black,draw=black,fill=up,rectangle,minimum height=1cm}}
\tikzset{view/.style={black,draw=black,fill=view,rectangle,minimum height=1cm}}
\tikzset{conv/.style={black,draw=black,fill=conv,rectangle,minimum height=1cm}}
\tikzset{bn/.style={black,draw=black,fill=bn,rectangle,minimum height=1cm}}

\newcommand*{\eg}{\emph{e.g.}\@\xspace}
\newcommand*{\Eg}{\emph{E.g.}\@\xspace}
\newcommand*{\ie}{\emph{i.e.}\@\xspace}
\newcommand*{\etc}{\emph{etc.}\@\xspace}
\newcommand*{\etal}{\emph{et al.}\@\xspace}
\newcommand*{\cf}{\emph{cf.}\@\xspace}
\newcommand*{\vs}{\emph{vs.}\@\xspace}
\newcommand{\KL}{\ensuremath{\mathrm{KL}}}
\newcommand{\Ber}{\ensuremath{\mathrm{Ber}}}
\begin{figure}
    \centering
    \begin{align}
        \theta \overset{G}{\rightarrow} \nu_\theta \overset{S}{\rightarrow} \phi_\theta \nonumber
    \end{align}
    \begin{tikzpicture}
    \node (p) at (0,0) {\includegraphics[width=2cm]{plots/forward.png}};
    \node[block, minimum width=2cm,rotate=90, label=left:G](G) at (2,0)  {Generator};
    \node[block,rotate=0, label=below:$\nu_\theta$](Vel) at (4,0)  {\includegraphics[height=1.5cm]{plots/TikzPictures/arrows.pdf}};
    \node[block, minimum width=2cm,rotate=90, label=left:S](S) at (6,0)  {Integration};
    \node[block, label=below:$\phi_\theta$](Phi) at (8,0)  {\includegraphics[height=1.5cm]{plots/TikzPictures/arrows2.pdf}};
    \node[above of = p, node distance =2cm] (theta) {$\theta$};
    \draw[->] (p) -- (G);
    \draw[->] (theta) -| (G);
    \draw[->] (G) -- (Vel);
    \draw[->] (Vel) -- (S);
    \draw[->] (S) -- (Phi);
    \end{tikzpicture}
    \caption{Process of generating a deformation field $\phi_\theta$ from the parameter vector $\theta$. The network-based \emph{generator} $G$ transforms the parameter vector into a \emph{velocity field} $\nu_\theta$. The \emph{solution operator} $S$ solves an associated flow equation, resulting in a final deformation $\phi_\theta$. Classically, the velocity field and the flow equation are formulated in Euclidean space; we extend the approach to the matrix group setting.}
    \label{fig:theta-to-phi}
\end{figure}

==> plots/TikzPictures/division-of-cube.tex <==



==> plots/TikzPictures/perceptron.tex <==
% \begin{figure}
%     \centering
%      \subfloat[]{\includegraphics[width=0.48\linewidth]{plots/MatrixInter.png}}
%      \subfloat[]{\includegraphics[width=0.48\linewidth]{plots/VecInter.png}}
%     \caption{The plot shows the convergence of the residual norm over the number of scaling-and-squaring steps for a given velocity field for a) the integration on SE(3) and b) the integration of a velocity field.}
%     \label{fig:scaling-squaring Convergence}
% \end{figure}
\begin{figure}[tb]
  \centering
  \hspace*{-0.75cm}
  \scalebox{0.87}{
  \begin{tikzpicture}
    \node (x) at (0,0) {$\begin{pmatrix}
        p_{i,1} \\
        p_{i,2} \\
        p_{i,3}
    \end{pmatrix}$};
 
    \node[conv,rotate=90,minimum width=4.5cm] (W1) at (1.25,0) {\small $\omega_0 W_1 \cdot + b_1$};
    \node[pool,rotate=90,minimum width=4.5cm] (sin1) at (2.5,0) {\small$\sin$};
    \node[conv,rotate=90,minimum width=4.5cm] (conv2) at (4.75,0)  {\small $W_2 \cdot + b_2$};
    \node[pool,rotate=90,minimum width=4.5cm] (pool2) at (6,0)  {$\sin$};
    \node (conv3) at (7.25,0) {$\oplus$};
    \node[conv,rotate=90,minimum width=4.5cm] (conv4) at (9,0)  {$W_6 \cdot + b_6$};
    \node (y) at (10.75,0) {$\begin{pmatrix}
        \nu_1(p_{i}) \\
        \nu_2(p_{i}) \\
        \vdots \\
        \nu_k(p_{i})
    \end{pmatrix}$};
    \node[draw,fill=gray, fill opacity=0.2, inner sep=4mm, label=below:4 times,fit=(conv2) (pool2) (conv3)] {};
    \node[draw,fill=blue, fill opacity=0.05, inner sep=10mm, fit=(x) (pool2) (y)] {};
    \draw[->] (x) -- (W1);
    \draw[->] (W1) -- (sin1);
    \draw[->] (sin1) -- (conv2);
    \draw[->] (conv2) -- (pool2);
    \draw[->] (pool2) -- (conv3);
    \draw[->] (sin1) -- (4 cm, 0) -- ++(0,2.5 cm) -| (conv3); 
    \draw[->] (conv3) -- (conv4); 
    \draw[->] (conv4) -- (y); 
    
  \end{tikzpicture}}
  \vskip 6px
  \caption{Network architecture of $G$ for generating the velocity field. The matrix-valued velocity field is described by a neural implicit representation that subsequently drives the evolution of a matrix field, generating a deformation.}
  \label{subfig:experiments-2d-architecture-vae}
\end{figure}




==> plots/TikzPictures/tables.tex <==
% \resizebox{10.5cm}{!}
% {\small
% \begin{tabular}{|p{4cm}||p{4cm}|p{4cm}|p{4cm}|}
%     \hline
%      \multicolumn{4}{|c|}{OASIS Brainscans (mean $\pm$ std)} \\
%      \hline
%      Method & Dice Score ($\uparrow$) & SSIM ($\uparrow$) & $\det(J_\phi)\leq 0$ ($\downarrow$)\\
%      \hline
%      initial & 0.5838 $\pm$ 0.0611 & 0.7347 $\pm$  0.0155  & \textbf{0}\\
%      SVF &  0.8090 $\pm$ 0.0255 & 0.9594 $\pm$ 0.0049 & $8.10\cdot10^{-6}$\\
%      SE3  & \textbf{0.8101 $\pm$ 0.0241}  & \textbf{0.9609 $\pm$  0.0047}  & $3.620\cdot10^{-5}$\\
%      Sim3 & 0.8092 $\pm$ 0.0260 & 0.9607 $\pm$ 0.0046 & $ 1.23\cdot10^{-5}$\\
%      SyN &  0.7816 $\pm$ 0.0340 & 0.896 $\pm$ 0.009  & \textbf{0}\\
%      \hline
%     \end{tabular}}
\resizebox{13.2cm}{!}
{\begin{tabular}{lllll} %
    \toprule
     %\multicolumn{4}{|c|}{OASIS: bidirectional comparison} \\
     %\hline
     method & Dice score $\pm$ std.~dev. ($\uparrow$) & Dice score backwards ($\uparrow$) & mean Dice score ($\uparrow$) & $\det(J_\phi)\leq 0$ ($\downarrow$)\\
     \hline
     initial  &  0.5838 $\pm$ 0.0610 & 0.5838 $\pm$ 0.0610 & 0.5838 $\pm$ 0.0610 &  - \\
     SVF \cite{han2023diffeomorphic} &   0.8153 $\pm$ 0.0231 & 0.8002 $\pm$ 0.0233 & 0.8077 $\pm$ 0.0223 & $2.35\cdot10^{-6}$ \\
     bidir. SVF &  0.8149 $\pm$ 0.0235 & \underline{0.8160 $\pm$ 0.0210} & \underline{0.8154 $\pm$ 0.02197} &  $3.58\cdot10^{-6}$ \\
     SE(3) [ours] & $\mathbf{0.8159 \pm  0.0231}$ & 0.8001 $\pm$  0.0233 & 0.8080 $\pm$ 0.0229 & $\mathbf{1.85\cdot10^{-6}}$\\
     bidir. SE(3) [ours] & 0.8148 $\pm$ 0.0238 & 0.8159 $\pm$ 0.0216 & 0.8153 $\pm$ 0.0224 & $2.90\cdot10^{-6}$\\
     SIM(3) [ours] & \underline{0.8157 $\pm$ 0.0233} & 0.8009 $\pm$  0.0233 & 0.8083 $\pm$ 0.0231 & $\underline{1.95\cdot10^{-6}}$\\
     bidir. SIM(3) [ours] &  0.8151 $\pm$ 0.0236 & \textbf{0.8162 $\pm$ 0.0212} & $\mathbf{0.8156 \pm 0.0221}$ & $3.20\cdot10^{-6}$ \\
     SyN \cite{avants2008symmetric} & 0.8062  $\pm$ 0.0248 & 0.8069 $\pm$ 0.0235  & 0.8066 $\pm$ 0.0241  &  $\mathbf{0}$\\
     \bottomrule
     \end{tabular}
}
